A Review of Deep Learning Techniques for Speech Processing

The field of speech processing has undergone a transformative shift with the advent of deep learning. The use of multiple processing layers has enabled the creation of models capable of extracting intricate features from speech data. This development has paved the way for unparalleled advancements in speech recognition, text-to-speech synthesis, automatic speech recognition, and emotion recognition, propelling the performance of these tasks to unprecedented heights. The power of deep learning techniques has opened up new avenues for research and innovation in the field of speech processing, with far-reaching implications for a range of industries and applications. This review paper provides a comprehensive overview of the key deep learning models and their applications in speech-processing tasks. We begin by tracing the evolution of speech processing research, from early approaches, such as MFCC and HMM, to more recent advances in deep learning architectures, such as CNNs, RNNs, transformers, conformers, and diffusion models. We categorize the approaches and compare their strengths and weaknesses for solving speech-processing tasks. Furthermore, we extensively cover various speech-processing tasks, datasets, and benchmarks used in the literature and describe how different deep-learning networks have been utilized to tackle these tasks. Additionally, we discuss the challenges and future directions of deep learning in speech processing, including the need for more parameter-efficient, interpretable models and the potential of deep learning for multimodal speech processing. By examining the field's evolution, comparing and contrasting different approaches, and highlighting future directions and challenges, we hope to inspire further research in this exciting and rapidly advancing field.

==> Sections/Application/s2s.tex <==
\subsection{Sequence to Sequence Models}
\label{sec:s2s}

The sequence-to-sequence (seq2seq) model in speech processing is popularly used for ASR, ST, and TTS tasks. The general architecture of the seq2seq model involves an encoder-decoder network that learns to map an input sequence to an output sequence of varying lengths. In the case of ASR, the input sequence is the speech signal, which is processed by the encoder network to produce a fixed-length feature vector representation of the input signal. The decoder network inputs this feature vector and produces the corresponding text sequence. This can be achieved through a stack of RNNs \cite{prabhavalkar2017comparison}, Transformer \cite{8462506} or Conformer \cite{gulati2020conformer} in the encoder and decoder networks.

The sequence-to-sequence model has emerged as a potent tool in speech translation. It can train end-to-end to efficiently map speech spectrograms in one language to their corresponding spectrograms in another. The notable advantage of this approach is eliminating the need for an intermediate text representation, resulting in improved efficiency. Additionally, the Seq2seq models have been successfully implemented in speech generation tasks, where they reverse the ASR approach. In such applications, the input text sequence serves as the input, with the encoder network creating a feature vector representation of the input text. The decoder network then leverages this representation to generate the desired speech signal.

\citet{karita2019comparative} conducted an extensive study comparing the performance of transformer and traditional RNN models on 15 different benchmarks for Automatic Speech Recognition (ASR), including a multilingual ASR benchmark, a Speech Translation (ST) benchmark, and two Text-to-Speech (TTS) benchmarks. In addition, they proposed a shared Sequence-to-Sequence (S2S) architecture for AST, TTS, and ST tasks, which is depicted in \Cref{fig:s2s}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{S2S.drawio.pdf}
    \caption{Unified formulation for Sequence-to-Sequence architecture in speech applications \cite{karita2019comparative}. $X$ and $Y$ are source and target sequences respectively.}
    \label{fig:s2s}
\end{figure}

\begin{itemize}
    \item Encoder
    \begin{equation}
    \begin{aligned}
        X_{0} &= \EncoderPreNet(X), \\
        X_{e} &= \EncoderMain(X_{0})
    \end{aligned}
    \end{equation}
    where $X$ is the sequence of speech features (e.g. Mel spectrogram) for AST and ST and phoneme or character sequence for TTS.
    \item Decoder
        \begin{equation}
        \begin{aligned}
        Y_{0}[1:t-1] &= \DecoderPreNet(Y[1:t-1]),\\
        Y_{d}[t] &= \DecoderMain(X_{e},Y_{0}[1:t-1]),\\
        Y_{post}[1:t] &= \DecoderPostNet(Y_{d}[1:t]),
        \end{aligned}
    \end{equation}
    During the training stage, input to the decoder is ground truth target sequence $Y[1:t-1]$. The Decoder-Main module is utilized to produce a subsequent target frame. This is accomplished by utilizing the encoded sequence $X_{e}$ and the prefix of the target prefix $Y_{0}[1: t-1]$. The decoder is mostly unidirectional for sequence generation and often uses an attention mechanism \cite{bahdanau2014neural} to produce the output. 
\end{itemize}

Seq2seq models have been widely used in speech processing, initially based on RNNs. However, RNNs face the challenge of processing long sequences, which can lead to the loss of the initial context by the end of the sequence \cite{karita2019comparative}. To overcome this limitation, the transformer architecture has emerged, leveraging self-attention mechanisms to handle sequential data. The transformer has shown remarkable performance in tasks such as ASR, ST, and speech synthesis. As a result, the use of RNN-based seq2seq models has declined in favour of the transformer-based approach. 

\subsubsection{Application}
Seq2seq models have been used for speech processing tasks such as voice conversion \cite{8683282,huang2019voice}, speech synthesis \cite{wang2017tacotron,wang2019deep,okamoto2019real,9003956,huang2019voice}, and speech recognition. The field of ASR has seen significant progress, with several advanced techniques emerging as popular options. These include the CTC approach, which has been further developed and improved upon through recent advancements \cite{graves2014towards}, as well as attention-based approaches that have also gained traction \cite{chorowski2015attention}. The growing interest in these techniques has increased the use of seq2seq models in the speech community.

\begin{itemize}
    \item Attention-based Approaches: The attention mechanism is a crucial component of sequence-to-sequence models, allowing them to effectively weigh input acoustic features during decoding \cite{bahdanau2014neural,luong2015effective}. Attention-based Seq2seq models utilize previously generated output tokens and the complete input sequence to factorize the joint probability of the target sequence into individual time steps. The attention mechanism is conditioned on the current decoder states and runs over the encoder output representations to incorporate information from the input sequence into the decoder output. Incorporating attention mechanisms in Seq2Seq models has resulted in an impressive performance in various speech processing tasks, such as speech recognition \cite{nankaku2021neural,prabhavalkar2017comparison,tuske2019advancing,weng2018improving}, text-to-speech \cite{shen2018natural,8682353,9053915}, and voice conversion \cite{8683282,huang2019voice}. These models have demonstrated competitiveness with traditional state-of-the-art approaches. Additionally, attention-based Seq2Seq models have been used for confidence estimation tasks in speech recognition, where confidence scores generated by a speech recognizer can assess transcription quality \cite{li2021confidence}. Furthermore, these models have been explored for few-shot learning, which has the potential to simplify the training and deployment of speech recognition systems \cite{higy2018few}.
    \item Connectionist Temporal Classification: While attention-based methods create a soft alignment between input and target sequences, approaches that utilize CTC loss aim to maximize log conditional likelihood by considering all possible monotonic alignments between them. These CTC-based Seq2Seq models have delivered competitive results across various ASR benchmarks \cite{higuchi2022bert,majumdar2021citrinet,synnaeve2020end,gulati2020conformer} and have been extended to other speech-processing tasks such as voice conversion \cite{zhang2019sequence,9362095,liu2021any}, speech synthesis \cite{zhang2019sequence} etc. Recent studies have concentrated on enhancing the performance of Seq2Seq models by combining CTC with attention-based mechanisms, resulting in promising outcomes. This combination remains a subject of active investigation in the speech-processing domain.
\end{itemize}
